Learning Transferable Adversarial Robust Representations via Multi-view Consistency

Despite the success on few-shot learning problems, most meta-learned models only focus on achieving good performance on clean examples and thus easily break down when given adversarially perturbed samples. While some recent works have shown that a combination of adversarial learning and meta-learning could enhance the robustness of a meta-learner against adversarial attacks, they fail to achieve generalizable adversarial robustness to unseen domains and tasks, which is the ultimate goal of meta-learning. To address this challenge, we propose a novel meta-adversarial multi-view representation learning framework with dual encoders. Specifically, we introduce the discrepancy across the two differently augmented samples of the same data instance by first updating the encoder parameters with them and further imposing a novel label-free adversarial attack to maximize their discrepancy. Then, we maximize the consistency across the views to learn transferable robust representations across domains and tasks. Through experimental validation on multiple benchmarks, we demonstrate the effectiveness of our framework on few-shot learning tasks from unseen domains, achieving over 10\% robust accuracy improvements against previous adversarial meta-learning baselines.

==> 7.reproducibility.tex <==
\clearpage
\section*{Reproducibility}

\begin{itemize}
    \item \textbf{Datasets.} We use CIFAR-FS, Mini-ImageNet, Tiered-ImageNet, CUB, Flower, and Cars for few-shot learning tasks. Further, we use CIFAR-10, CIFAR-100, STL-10 for standard image classification tasks in transfer learning. More details are in Supplementary~\ref{appendix:dataset}.
    
    \item \textbf{Meta-train.} We trained our models on CIFAR-FS and Mini-ImageNet with ResNet12 and ResNet18 as the base encoder. All models are trained on 5-way 5-shot support set images and 5-way 15-shot query images. More details are in Supplementary~\ref{appendix:meta-train}.
    
    \item \textbf{Meta-test.} We evaluate our models on few-shot learning tasks as described in Supplementary~\ref{appendix:meta-test}. For adversarial setting for few-shot robustness is written in Supplementary~\ref{appendix:adv}.
    
    \item {\textbf{Table~\ref{table:cifar-crossdomain},~\ref{table:mini-crossdomain},~\ref{table:baseline_result}.}} Please see Section~\ref{sec:adv_fewshot} and Supplementary~\ref{appendix:meta-train},~\ref{appendix:meta-test} to reproduce the results in those Table.
    
    \item{\textbf{Table~\ref{table:metamodel-agnostic},~\ref{table:meta_architecture_cross_domain}.}} Please see Section~\ref{sec:adv_fewshot} to reproduce the results, and more details for hyperparameters are in Supplementary~\ref{appendix:hyper-metaleaning}. For adversarial setting, see Supplementary~\ref{appendix:adv}.
    
    \item{\textbf{Table~\ref{table:compareAug}.}}  Please see Section~\ref{section:compareAug} and Supplementary~\ref{appendix:aug} to reproduce the Table~\ref{table:compareAug}. Detailed algorithm for bilevel parameter augmentation and image-only augmentations we utilized are described in Algorithm~\ref{algo:algorithm} and Algorithm~\ref{algo:algorithm_img}, respectivley.
    
    \item{\textbf{Table~\ref{table:compareAttack}.}} Please see Supplementary~\ref{appendix:bilevelattack} to reproduce the Table~\ref{table:compareAttack}. Bilevel attack is explained in Section~\ref{sec:bilevelattack},~\ref{section:bilevel_ablation}.
    
    \item{\textbf{Table~\ref{table:table_transfer},~\ref{table:table_transfer_others},~\ref{table:selfsup_loss_ablation_full}.}} Please see Supplementary~\ref{appendix:selfsup} to check the baselines, and see Supplementary~\ref{appendix:self-sup_rft} to reproduce the results.
    
    \item{\textbf{Table~\ref{table:compareAug_Cross}.}} Please see Supplementary~\ref{appendix:meta-objective} to reproduce the results.
    
    \item{\textbf{Table~\ref{table:common_corruption}.}} Please see Supplementary~\ref{appendix:transfer} to reproduce the results.
    
    \item{\textbf{Table~\ref{table:rocl}.}} Please see Supplementary~\ref{appendix:rocl} to reproduce the results.
    
    \item{\textbf{Table~\ref{table:obfuscated}.}} Please see Supplementary~\ref{appendix:obfuscated} to reproduce the results.
    
    \item{\textbf{Figure~\ref{fig:loss_surface},~\ref{fig:loss_surface_unseen}.}} Please see Supplementary~\ref{appendix:loss_surface} to reproduce the results.
    
    \item{\textbf{Figure~\ref{figure:cka_aug},~\ref{figure:cka_attack}.}} Please see Supplementary~\ref{appendix:cka} to reproduce the results.
\end{itemize}

==> Deleted_intro.tex <==
\section{Introduction}
The ability to rapidly adapt to a new task with only a small amount of data is a fundamental aspect of artificial general intelligence. To achieve this, meta-learning~\citep{thrun1998learning} has been proposed to learn to learn a new task quickly with limited data with deep neural networks (DNNs)~\citep{koch2015siamese, sung2018learning, snell2017prototypical, finn2017model, nichol2018first}. However, meta-learners based on DNNs can be easily deceived by small imperceptible perturbations to the input data~\citep{szegedy2013intriguing}.

To overcome such adversarial vulnerability of DNN meta-learners, several existing works~\citep{yin2018adml, goldblum2020adversarially, wang2021rmaml} have proposed to train adversarially robust meta-learners by simply combining task-dependent class-wise attacks from adversarial training (AT)~\citep{madry2017pgd} with meta-learning approaches~\citep{finn2017model}. 
However, we find that these approaches are only effective in achieving robustness to perturbations from a seen domain, while showing poor transferable robustness to unseen domains as shown in Table~\ref{table:cifar-crossdomain}. Since they utilize \textit{task-dependent adversaries}, they have difficulty adapting to novel tasks from unseen domains, which is a crucial challenge of meta-learning for its real-world applications. 
In the unseen domain, the task-dependent adversarial perturbations could not learn robust unseen representation, leading to a significant overlap in the latent representations of attacked samples across different classes of unseen tasks (Figure~\ref{fig:tsne_aq}). Further, this overlap demonstrates that solely adapting the classifier in a specific task is not enough to correctly predict. Thus, in order for a meta-learning framework to be robust to such challenging settings, not only the classifier, but the representations should be robust to unseen tasks and domains, which can be achieved through employing task-agnostic adversaries.


\input{Figure/Captions/concept_fig_baseline.tex}
To this end, we propose a novel meta-adversarial learning framework that focuses on learning transferable robust representations, \textit{\textbf{M}eta-\textbf{A}dversarial Multi-\textbf{V}iew \textbf{R}epresentation \textbf{L}earning} (\textbf{MAVRL}) (Figure~\ref{fig:concept_figure}). Specifically, we employ a multi-view representation learning framework by proposing multi-view inner adapted encoders from the same meta-initialized parameters. Then we meta-learn these multi-view encoders with a bilevel optimization scheme which consists of an inner optimization step for generating different views of the same input image, and an outer meta-optimization step for meta-learning the robust representations for unseen tasks and domains. 

During the inner adaptation step, we adapt the encoder for each view by updating its parameters by taking gradient steps with two different sets of augmentations for the same support set images. Such augmentation and update of the multi-view encoders allow the model to generate diverse multi-view latent features even in a few-shot learning scenario. Then, at the outer meta-optimization phase, we apply a novel task-agnostic adversarial attack in the latent space that does not require any labels, which aims to maximize the discrepancy across the latent features encoded by the two different views. Finally, we explicitly minimize the representational discrepancy across clean and perturbed samples on another batch of images for unseen tasks. This adversarial meta-learning of the multi-view encoders with latent feature attacks allows us to learn latent representations across different batches of images, thereby obtaining a more discriminative space even for images from unseen domains (Figure~\ref{fig:tsne_ours}).


To verify the efficacy of our robust representation learning scheme, we meta-learn the framework on the source domain (CIFAR-FS, mini-ImageNet) and validate its robustness on unseen domains such as CUB, Flower, Cars, and Tiered-ImageNet. Overall, our novel approaches can consistently and significantly improve the robustness compared to the previous adversarial meta-learning methods~\citep{yin2018adml, goldblum2020adversarially, wang2021rmaml}. In particular, our method improves few-shot clean and robust classification accuracy on unseen Tiered-ImageNet from 29.54\% $\rightarrow$ 51.46\%, and 9.30\% $\rightarrow$ 30.06\% against adversarial attack~\citep{madry2017pgd}, respectively. Furthermore, visualization of the loss surface also verifies that our model learns robust representation that can be easily transferred to different domains (Figure~\ref{fig:loss_surfaces}).

To summarize, our contributions are fourfold as follows:
\begin{tcolorbox}[enhanced,attach boxed title to top center={yshift=-3mm,yshifttext=-1mm},
  colback=blue!5!white,colframe=blue!75!black,colbacktitle=red!80!black]
\begin{itemize}[leftmargin=*]
\item We tackle a crucial problem in the field of meta-adversarial learning, specifically the \textbf{transferability of the robustness across unseen tasks and domains with limited data}, which is an ultimate goal of meta-learning framework for real-world application, yet has been under-explored in previous studies.

\item We propose a \textbf{novel multi-view robust representation learning framework}, which adversarially meta-learns the multi-view encoders that the representations from the two views adapted to different augmentations of the same support images with task-agnostic adversarial attacks.

\item To adversarially train the multi-view encoders, we propose a novel task-agnostic adversarial attack that aims to maximize the \textbf{representational discrepancy} across the views.

\item Our framework obtains impressive transferable robustness on few-shot tasks from unseen domains. Notably, our model outperforms baselines by \textbf{more than 10\%} in robust accuracy without compromising clean accuracy.
\end{itemize}
\end{tcolorbox}



==> Figure/Captions/cka_analysis.tex <==
\begin{wrapfigure}[18]{r}{0.4\textwidth}
\centering

\end{wrapfigure}

==> Figure/Captions/concept_baselines.tex <==
\begin{figure}
     \centering
     \begin{subfigure}[b]{0.18\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figure/maml_concept.png}
         \caption{MAML}
         \label{fig:maml}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.28\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figure/aq_concept.png}
         \caption{AQ}
         \label{fig:aq}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.52\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figure/our_concept.png}
         \caption{Ours}
         \label{fig:our_concept}
     \end{subfigure}
        \caption{\textbf{Comparison of our concept with other meta-learning frameworks.} All three models have two optimizations: inner and outer optimization. MAML updates the parameters of both the encoder and classifier in the inner loop. AQ uses a solver as a classifier to calculate the solution of query set images based on support set images in the inner loop and construct adversarial examples with class-wise attack. Unlike previous works, our model only updates the encoder parameters in the inner loop. Especially, we propose two-level augmentation to effectively construct adversarial images coined with instance-wise dynamic attack which does not require any labels.}
        \label{fig:three_concept}
       
\end{figure}
%aq gradient 방향이 \theta_i 에서 \theta로 가야하는거 아닌가?

==> Figure/Captions/concept_fig_baseline.tex <==
\begin{figure}[t]
    \centering
    \begin{minipage}[t]{0.4\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figure/concept_fig_1.pdf}
        \caption{Conventional Adversarial Meta-Learning}
        \label{fig:concept_subfig1}
    \end{minipage}\hfill
    \begin{minipage}[t]{0.6\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figure/concept_fig_2.pdf}
        \caption{Our Multi-view Adversarial Meta-Learning}
        \label{fig:concept_subfig2}
    \end{minipage}
\caption{\small \textbf{Overview of MAVRL.} (a) Conventional adversarial meta-learning approaches aim to enhance the robustness of the model by simply incorporating conventional adversarial training schemes (i.e., class-wise attack) into meta-learning frameworks. Since they mostly meta-learn the classifier (i.e., $h(\mu)$) and generate task-dependent adversaries, they have difficulties generalizing to unseen domains. (b) MAVRL focuses on meta-learning the representations, rather than classifiers, that are transferably robust across tasks and domains. Specifically, MAVRL meta-learns the Siamese encoders, in which the encoder for each view (i.e.,$f(\theta_1^{\tau}), f(\theta_2^{\tau})$) are separately adapted to different augmentations of the same support set, to minimize the loss on \textit{multi-view latent attacks} for unseen queries. The multi-view latent attacks are novel unsupervised adversarial attacks that aim to maximize the representational discrepancy across the views.}
\label{fig:concept_figure}
\end{figure}

==> Figure/Captions/loss_surface_unsee.tex <==
\begin{figure}[t]
    \centering
    \begin{minipage}[t]{0.45\linewidth}
        \centering
        \includegraphics[width=0.9\linewidth]{Figure/aq_clean_mini.png}
        \subcaption{AQ}
        \label{fig:loss_unseenmini_subfig1}
    \end{minipage}\hfill
    \begin{minipage}[t]{0.45\linewidth}
        \centering
        \includegraphics[width=0.9\linewidth]{Figure/marvl_clean_mini.png}
        \subcaption{MAVRL}
        \label{fig:loss_unseenmini_subfig2}
    \end{minipage}
    \caption{\small Loss surface of the unseen domain (Mini-ImageNet)}
    \label{fig:loss_surface_unseen}
\end{figure}


==> Figure/Captions/model_figure.tex <==
\begin{figure*}
\centering{
\includegraphics[width=\textwidth]{Figure/model_figure.png}
}
\vspace{-0.2in}
\caption{\small \textbf{Model figure.} \textit{}}
\label{fig:model_figure}
\vspace{-0.2in}
\end{figure*}


==> Figure/Captions/selfsup_vs_ours.tex <==
\begin{wrapfigure}[9]{r}{0.45\linewidth}
\vspace{-0.2in}
\centering
    \includegraphics[width=0.9\linewidth]{Figure/selfsup_vs_ours.pdf}
\vspace{-0.07in}
\caption{\small A graphical illustration of our motivation for multi-view instance-attack.}
\label{fig:selfsup_vs_ours}
\end{wrapfigure}

==> Response.tex <==
\section*{R1 (4)}
\paragraph{Summary}
1. Concept Figure 1 (a) is hard to comprehend: Figure 1 (a) represents previous adversarial meta-learning, that simply combines meta-learning and adversarial training. We revise Figure 1 in the \href{https://drive.google.com/drive/folders/1avD6Q2NYK2PEyxbdMbe2uTqQdUUiNer5?usp=share_link}{anonymous link}.
2. Multi-view is a basic form of data augmentation which is lack novelty: This is a factual misunderstanding of our multi-view encoder augmentation. Multi-view encoder augmentation is a novel approach that employs meta-encoders in the inner adaptation of the meta-learning framework as a multi-view generator.  
3. Absence of ablation study of loss function: We provide loss ablation in Figure 5, augmentation ablation in Table 5, and attack ablation in Table 6 in the main manuscript.
4. Real training data experiment is needed: We provide additional real training data experiments and also experiment on the realistic dataset in the response.
Detailed responses are in the following threads.

\subsection{1. Concept Figure is hard to comprehend}
\paragraph{Review:} The visualization of Fig.1, particularly Fig.1(a), appears to be complex and challenging to comprehend.
\paragraph{Answer: } We clearly note that Fig.1 (a) is not our approach, but is previous conventional adversarial meta-learning which is a simple combination of meta-learning and adversarial learning. Meta-learning consists of bi-level optimization; inner adaptation and outer meta-optimization. During the inner adaptation phase, the meta-learner obtains task-adaptive parameters ($\mu^\tau$) with clean support set images and then utilizes those parameters to optimize the meta-objectives ($\Lagr$) against perturbed query set images in the meta-optimization phase. Adversarial training consists with the min-max optimization, where attacked examples are generated by maximizing the cross entropy loss of the images based on labels (red outlined image: dog) while utilizing those attacked images to minimize the training loss. To clarify the concept, we revise Figure 1 as shown in the \href{https://drive.google.com/drive/folders/1avD6Q2NYK2PEyxbdMbe2uTqQdUUiNer5?usp=share_link}{anonymous link} that is more simplified and also compare with the clean meta-learning. Additionally, we describe our novel approaches in the following question.

\subsection{2. Multiple-views in this work seems basic form of data augmentation: lack novelty}
\paragraph{Review:} The utilization of multiple views in this work seems to be a basic form of data augmentation, lacking novelty.
\paragraph{Answer: } We would like to clarify that our multiple views augmentation is beyond basic data augmentation which is uniquely defined with the bi-level meta-learning. During the inner adaptation phase, our approach generates multi-view Siamese encoders with task and view-adaptive parameters using data-augmented support set images and uses those multi-view encoders to generate adversaries that aim to maximize the discrepancy. Then, we learn robust representations by enforcing agreement between two views of robust latent with the similarity loss and explicitly regularize each latent to be robust with the adversarial loss in the meta-optimization phase. This novel approach enables learning transferable robust representation to unseen domains and tasks. Moreover, the multi-view representation learning framework has not been introduced in either meta-learning or self-supervised learning before, demonstrating its novel contribution. 


%$    - Our multiple view is not a basic form of data augmentation.
%    - First of all, our multiple-view is not a basic form of data augmentation. While two views are generated from different transformation

\subsection{3. Absence of ablation study}
\paragraph{Review:} The absence of ablation studies investigating the impact of different loss functions is a notable limitation of the study, which is arguably its main contribution.

\paragraph{Answer:} We demonstrate the effectiveness of the proposed meta-objectives in Figure 5, where our meta-objective notably achieves superior robustness on unseen domains and tasks. Specifically, our meta-objective consists of two terms, adversarial loss and similarity loss, where adversarial loss aims to learn robust representation and similarity loss enables learning view-invariant representations, respectively. As shown in Figure 5, the model trained with each loss alone shows poor performance. 

\subsection{4. Loss ablation is needed}
\paragraph{Review:} It would be beneficial to include ablation studies regarding the impact of different loss functions in the proposed method, as this would provide valuable insights into the contributions of each component and improve the interpretability of the results.
\paragraph{Answer: } We included loss function ablation in Figure 5, augmentation ablation in Table 5, and attack type ablation in Table 6. The loss function ablation demonstrates that the similarity loss between different view latents is the influential factor for robust generalization (Line 413).

Following question 5, we had ablation experiments on loss function in Figure 5. Especially, we demonstrate that the similarity loss between different view latents is the influential factor to achieve transferable robust representations on unseen domains (Line 413). Further, we also demonstrate the contributions of each component such as augmentation (Figure 6, Table 5) and attack (Figure 6, Table 6) through ablation studies. 

\subsection{5. [Experiment] Real training data experiment is needed}
\paragraph{Review:} The current amount of training data provided in the study may not be sufficient to fully showcase the capabilities of the proposed method and could potentially be interpreted as a form of data augmentation rather than true Multiview learning. Therefore, additional real training data examples could be included in this paper to better demonstrate the effectiveness of the proposed approach in capturing diverse representations and improving performance.
\paragraph{Answer: } 
First of all, our approach is not multi-view learning but meta-adversarial learning coined with multi-view representation learning. To recap our approach, we generate multi-view encoders to maximize the discrepancy between two different latents in the inner adaption phase while maximizing the agreement between two views to learn transferable robust representations in the meta-outer optimization phase, which is a novel framework to achieve robust generalization in the meta-learning. Existing meta-adversarial learning approaches validate their method on few-shot benchmark datasets (CIFAR-FS, Mini-ImageNet, Tiered-ImageNet, CUB, Flower, and Cars) as done in the main paper (Table 1 and 2); however, based on your concerns, we have conducted experiments on additional real data with full classes, CIFAR-10, CIFAR-100, EuroSAT, and ISIC, which have 10, 100, 7, and 7 classes, respectively, in the following table. Especially, since our pre-trained meta-learner is trained on CIFAR-FS with few-shot classification tasks, we adopt robust full-finetuning which is widely used in validating self-supervised learning approaches. Our model is trained with our multi-view representation learning shows superior robustness and transferability even on standard classification tasks against realistic datasets with full classes as well as few-shot classification tasks, which outperforms the model trained with only data augmentation demonstrating the effectiveness of our methods.

% evaluation on full-dataset with robust full-finetuning
|                | CIFAR-10  |           | CIFAR-100     |           | EuroSAT   |           | ISIC   |           |
|----------------|-----------|-----------|---------------|-----------|-----------|-----------|-----------|-----------|
|                | Clean     | PGD       | Clean         | PGD       | Clean     | PGD       | Clean     | PGD       |
| Data Aug.      | 66.79     | 44.32     | 38.49         | 22.21     |      |      |      |      |
| Multi-view Aug.| 67.25     | 44.63     | 36.37         | 22.43     |      |      |      |      |

% train on full-dataset of cifar-100

\section*{R2 (6)}
\paragraph{Summary}
1. AT vs meta AT requires more time cost: we compare the computational cost in the table.
2. the effectiveness of the data augmentation in MAVRL: We conduct additional ablation on different types of augmentation, such as simple augmentation, or randAug, etc, in the response.
3. Visualization on the different datasets: We visualize on general dataset, CIFAR-10, and fine-grained dataset, CARS, and Flowers in the \href{https://drive.google.com/drive/folders/11eXgUtoZkLGP5ZajFKIBwl5R-GwN_Y9l?usp=share_link}{anonymous link}.
Please find the detailed response in the following thread.

\subsection{1. AT vs meta AT requires more time cost}
\paragraph{Review:} Compared with traditional adversarial training, the meta-training procedure requires much more training cost to improve robust performance.
\paragraph{Answer: } It is important to note that meta-adversarial training targets robust few-shot learning, which is a different research area compared to traditional adversarial training. Although comparing the two directly is not a fair comparison, we provide a table comparing the number of training samples required for robust prediction and the cost of computation. We hope this table helps clarify the differences between the two approaches.
% - Adversarial training from scratch (# of training samples & training cost) vs ours

% | Model | Learning type | # of training samples per iteration | # of training classes | total epochs | Training time (s/epoch) |
% |------------------|:----------:|:--------------:|:----------:|:--------------:|:----------:|
% | TRADES | Adversarial learning |  batch size  | 100 | 110 | 233s |
% | MAVRL  | Meta-adversarial learning | batch size * (5-way 5-shot support set & 5-way 15-shot query set) | 80 | 300 | 600s |


\subsection{2. [Experiment] Affect of different kinds of data augmentation? }
\paragraph{Review: } How do different kinds of data augmentation affect the final performance? In Table 5, we can only tell that the data augmentation and multi-view augmentation play a positive role in the robustness. More details are encouraged to verify the effectiveness of the data augmentation in MAVRL.
\paragraph{Answer: } Thanks to your comments, we performed four kinds of augmentation ablation experiments, 1) no data augmentation, 2) simple data augmentation (random crop, horizontal flip), 3) ours and 4) RandAug~\citep{cubuk2020randaugment} to verify how the different kinds of data augmentations affect to our methods. The results show that while data augmentation plays a positive role in robustness, our multi-view augmentation consistently boosts the robustness even further. Our data augmentation techniques contains random crop, color jitter, horizontal flip, grayscale, and solarization, as used in \citet{zbontar2021barlow}. 
%- single view, different augmentation

\subsection{3. [Experiment] Visualization on different dataset (More fine-grained dataset)}
\paragraph{Review: } In Figure 4, the representations of the data in different classes on the unseen domain are clearly separated. However, the selected classes in Cifar10 are quite different, which is hard to verify the transferability of the MAVRL in the fine-grained level. It is better to provide the visualization on some similar unseen classes for evaluation.
\paragraph{Answer: } We have added visualizations on the Flowers and Cars datasets in the \href{https://drive.google.com/drive/folders/11eXgUtoZkLGP5ZajFKIBwl5R-GwN_Y9l?usp=share_link}{anonymous link} which are fine-grained datasets. The visualizations demonstrate that the transferability of MAVRL in fine-grained level by showing well-separated robust embedding compared to baseline.

\section*{R3 (4)}
\paragraph{Summary}
1. Notation is not well organized \& problem setting is not well organized: We re-emphasize our problem setting more precisely in the response. Please find our response.
2. Learning framework is confusing: We explain our framework more clearly in the response. We also illustrate our approach more simple and clear in the \href{https://drive.google.com/drive/folders/1avD6Q2NYK2PEyxbdMbe2uTqQdUUiNer5?usp=share_link}{anonymous link}. Please find our additional figure to help your understanding.
3. Explanation of the insights is lack: We explain our insights more clearly in the response. We would like to clarify that our approach is not a combination of contrastive learning and meta-adversarial training. Our approach does not use contrastive learning.

\subsection{1. Notation is not well organized \& problem setting is not well organized}
\paragraph{Review: } The notations in this paper are not well-organized. Some notations lack explanations and some are abused. For example, $S\tau$ denotes support set in the problem setting while denotes multi-view support set in later context.
The statement of problem setting is not well-organized and some polish work is required.
\paragraph{Answer: } We will revise and clarify the notations in the paper. In particular, $S_\tau = {x^s, y^s}$ denotes the support set in the meta-learning framework, and it has a consistent meaning throughout the paper. Thus, we will denote the multi-view support set as $S'_\tau = {t_1(x^s), t_2(x^s), y^s}$ with differently transformed. We will ensure that the explanations for each notation are provided precisely as you commented.

\subsection{2. Learning framework is confusing}
\paragraph{Review:} The proposed learning framework is not well stated and is confusing. For details, please refer to Q4 in Question part.
\subsection{Q4. Is the method based on a pre-trained backbone?}
\paragraph{Review: } Is the proposed method based on a pre-trained backbone? I am not sure about this since both context and algorithm table don’t mention this but the illustration figure contains a backbone before the two SSL backbone. If yes, how does the optimization process work?

\paragraph{Answer: } No, our method does not use any type of pre-training backbone. Our approach is a meta-adversarial learning framework to learn robust representations that can be easily transferred to unseen domains. To achieve this, we introduce the concept of augmenting the encoders into multi-view Siamese encoders (green and purple encoders in Figure 1 (b)) during inner adaptation in meta-learning, which maximizes the discrepancy between two views, preventing them from representation collapse. Then, in the outer optimization, we explicitly optimize the meta-learner (blue encoder in Figure 1 (b)) to minimize the robust loss and also discrepancy between the two views against other tasks, which helps learn transferable robust representation on unseen domains. Here, the blue encoder is not a SSL backbone, but a meta-initialized encoder that ultimately learns the meta-knowledge in the meta-optimization phase.

% Our approach is a novel multi-viewed meta-adversarial learning framework, which is not a simple combination of meta-learning, adversarial attack, and contrastive learning. Furthermore, we do not exploit contrastive learning anywhere. Our goal is to learn robust meta-knowledge that can be transferred to unseen domains. To achieve this, we introduce the concept of augmenting the encoders into multi-view Siamese encoders during inner adaptation in meta-learning, which helps learn robust representations that are not dependent on label information. Then, in the outer optimization, we explicitly optimize the meta-learner to minimize the robust loss and also discrepancy between the two views.


%Our framework is basically meta-learning framework which bilevel optimization which compose with inner adaptation (Grey box in Figure 1 (b)) and outer optimization (Yellow box in Figure 1 (b)). To obtain robustness, we employ adversarial examples (red outlined dog images) in the outer optimization. Until this framework, it is same as conventional adversarial meta-learning (Figure 1 (a)). However, conventional adversarial meta-learning approaches are not robust in the unseen dataset which is not transferable robustness. To overcome such limitation, we propose multi-view latent attack which generate adversaries that helps to learn generalized robust representation in the outer-optimization. To generate multi-view latent attack, we propose multi-view augmentation in the inner adaptation which is firstly propose that augment the encoders it-selves with the differently augmented support sets (green: view 1 dog image and puple: view 2 dog image) in the inner adaptation, please note that it is not a simple data augmentation. By employing multi-view augmented encoders, we generate more diverse and effective adversaries that maximize the discrepancy of each latent from multi-view encoders (Multi view latent attack transparent pink box). Then, we train to maximize the similarity between adversaries and clean images in the outer optimization. 

\subsection{3. Explanation of the insights are lack}
\paragraph{Review:} The explanations of the insights behind the proposed method lack. Thus, the proposed method looks like a simple combination of meta-learning, adversarial attack and contrastive learning. Besides, conventional contrastive learning tries to learn a single backbone by applying tricks on Siamese networks, but the proposed method preserves the two sub-networks. So, it is not convincing whether the MAVRL learns good representations.
% \paragraph{Answer:} First of all, we want to clarify that our approach is a novel multi-viewed meta-adversarial learning framework that has never been introduced, and we do not utilize contrastive loss anywhere in our framework, which is not a simple combination of meta-learning, adversarial attack, and contrastive learning. Moreover, the previous meta-adversarial learning which is a simple combination of meta-learning and adversarial learning is described in Figure 1(a), and our novel multi-viewed meta-adversarial learning framework is demonstrated in Figure 1(b). Our ultimate goal is to obtain robust meta-knowledge which can be transferred to unseen domains while previous work extremely breaks down to unseen domains (Table 1,2). To obtain generalized robust meta-knowledge, we employ adversarial examples that do not rely on label information and do not relevant to each task by using multi-view latent spaces. Specifically, we generate adversaries by maximizing the discrepancy between two views from multi-view encoders while enforcing consistency on two robust representations and explicitly regularizing adversarial loss to achieve robust generalization. As shown in the visualization of the embeddings (Figure 4), MAVRL learns good robust representations on CIFAR-10, which is an unseen domain against CIFAR-FS. Additionally, we visualize the embeddings on the fine-grained datasets (Cars and Flower) which have a more different distribution from the train dataset (CIFAR-FS), also achieving well-separated robust representations while existing meta-adversarial work shows overlapped embeddings.

The main insights are based on the limitation of existing conventional meta-adversarial learning approaches (Figure 1(a)) that are actually a simple combination of meta-learning and adversarial attacks, which are extremely vulnerable to unseen domain tasks as shown in Table 1 and 2. This is because they only reuse the representation without focusing on representation learning, thus existing approaches are only effective on unseen domains that have a highly similar distribution to seen domain [1]. To overcome such restricted transferable robustness, we propose novel meta-adversarial learning to learn a robust representation that can be generalized to unseen domains via multi-view representation learning. We clearly note that our approach is not a simple combination of meta-learning, adversarial attack, and contrastive learning. We recap our main contributions as follows:
1. Our primal focus is on robust representation learning to enable transferring learned representations to unseen domains.
   Since conventional meta-adversarial learning approaches are based on representation reuse schemes without focusing on representation learning, they extremely break down to the unseen domain tasks that have a highly different distribution from source domains as demonstrated in [1] and Table 1 in the main paper. However, we mainly focus on representation learning coined with the bilevel optimization scheme, which enables learning transferable robust representations demonstrating the superior ability to be generalized on unseen domains.
2. We introduce multi-view augmentation that can effectively prevent representation collapse for the meta-learning framework.
    In self-supervised learning (SSL) approaches, the effectiveness of utilizing multiple views is already demonstrated in terms of achieving generalization. Especially, conventional SSL methods adopt additional networks [2], or regularization methods [3] to prevent representation collapse between different views. However, we propose a multi-view augmentation that enables avoiding representation collapse without any additional components via meta-learning. Specifically, we generate multi-view encoders with task-specific parameters during the inner adaptation phase, which can maximize the discrepancy between two views. 
The proposed learning framework has never been introduced in meta-learning, adversarial learning, and self-supervised learning, demonstrating the novelty of our work. With the above two main contributions, MAVRL can learn robust representations that can be easily transferred to unseen domain tasks, outperforming conventional meta-adversarial learning by more than 10\% of robustness. Moreover, we do not exploit contrastive learning anywhere in our framework, it is totally misunderstanding. 

[1] Oh, Jaehoon, et al. "Boil: Towards representation change for few-shot learning." ICLR 2021
[2] Zbontar, Jure, et al. "Barlow twins: Self-supervised learning via redundancy reduction." International Conference on Machine Learning. PMLR, 2021
[3] Bardes, Adrien, Jean Ponce, and Yann LeCun. "Vicreg: Variance-invariance-covariance regularization for self-supervised learning." ICLR 2022

% our insights is that we need to employ adversaries examples which can lead us to learn robust representation which is not dependent on label information especially dependent to each task. Therefore, we introduce to utilize unlabeled attack but to maximize the effectiveness of unlabeled attack, data augmentation itself is limited function to form enough diverse view when the data is very limited in meta-learning. Therefore, we propose novel concept of augmenting the encoders during the inner adaptation.

\subsection{4. Why the computation overhead is reduced in Meta-SGD?}
\paragraph{Review: } The explanation of X and Y lacks. I think $Y\tau$ can be explained as the ‘the corresponding labels of $X\tau$’ instead of ‘a set of classes’. Line 233-236 left side mentions that meta-learning $\alpha$ helps reduce the computation overhead. As far as I know, meta-learning $\alpha$ requires further calculation of gradients of $\alpha$. So, why the computation overhead is reduced?
\paragraph{Answer: } As you commented, X is the image and Y is the corresponding class label, but "set of the classes" is also the right expression. $X^\tau$ and $Y^\tau$ are denoted to discriminate task ($\tau$) in the few-shot meta-learning setting (Line 152). 

In MAML, $\alpha$ is a scalar value to calculate gradients in the inner adaptation of meta-learning, so MAML needs several steps in the inner adaptation. In Meta-SGD, $\alpha$ is a learnable vector, which is trained during meta-learning. Therefore, Meta-SGD does not need to take several gradient steps during inner adaptation, which eventually reduces the computation overhead [1].
[1] MetaSGD

\subsection{5. Does this approach benefits from proposed framework or from using more parameters?}
\paragraph{Review: } Contrastive learning framework aims to learn a single backbone that can perform well on downstream tasks by applying tricks, such as gradient stop, to Siamese encoders. In this paper, a Siamese encoder is also adopted yet seems to preserve both sub-networks. So, whether the framework works or the more parameters work?

\paragraph{Answer: } Our framework does not use more parameters. Multi-view augmented encoders are generated on the fly during the inner adaptation phase of the meta-learning (Line 172), and only the meta-initialized encoder ($\theta$) is eventually trained in the meta-optimization phase as other meta-learning method works. Our framework generates effective adversaries using proposed multi-view encoders by maximizing the discrepancy between different view latents and explicitly meta-optimizing to minimize the vulnerabilities between unseen tasks. Our primary focus is to learn generalized robust representations using multi-view augmented encoders in the meta-learning framework, not contrastive learning, and even we do not utilize contrastive loss anywhere in our framework. The Siamese encoders are instrumental in our meta-learning framework to generate multi-view latent and it is essential to achieve robustness in unseen tasks.


\paragraph{global comment}
To provide clarity to reviewers, we would like to highlight our main contributions. Our ultimate goal is to learn robust representations that can be easily transferred to unseen domains through meta-learning. To achieve this goal, we propose a novel meta-adversarial learning framework along with multi-view representation learning.

Specifically, our contributions are as follows:

1. We introduce robust representation learning using the bilevel meta-learning framework for transferable robustness on unseen domains. This is totally different from previous meta-adversarial learning methods, which primarily focus on learning the optimal weight of the final classifier and reusing the representation.
2. We propose a novel multi-view augmentation via inner adaptation of meta-learning, which naturally prevents representation collapse by maximizing the discrepancy between two views, without the need for additional networks or regularization.


\section{AC Letter}
Dear AC, SAC, and PCs,
We deeply appreciate your time and effort in meta-reviewing our paper.

We tackle the practical problem of achieving transferable robustness on unseen domains with much fewer examples. To resolve such an important yet under-explored problem, we propose a novel meta-adversarial learning framework that learns transferable robust representation which could be generalized to unseen domains via multi-view representation learning. Specifically, to learn transferable robust representations, we generate multi-view encoders with view- and task-adaptive parameters to maximize the discrepancy between different latents during the inner adaptation while minimizing the discrepancy between two attacked latent and explicitly regularizing them to be robust on unseen tasks in the meta-optimization phase. Extensive experimental results demonstrate the effectiveness of our approaches, outperforming baselines by more than 10\% of improvements in robustness against unseen domain tasks.

Despite the novel approach for unseen robustness of few-shot tasks, Reviewer bZs8 gave us a rating of borderline reject based on the main concern that the proposed method is a simple combination of meta-learning, adversarial attack, and contrastive learning. However, this is a critical misunderstanding, since we do not exploit the contrastive learning anywhere in our framework, and even we describe conventional meta-adversarial learning that is a simple combination of meta-learning and adversarial learning in Figure 1 (a), which is completely different from our framework (Figure 1 (b)). Moreover, we presume that Reviewer bZs8 lacks basic knowledge of the meta-learning to properly review our paper, asking the reason why Meta-SGD can reduce the computational overhead, and whether the performance improvements are due to an increased number of parameters obtained during the inner adaptation of the meta-learning, which is based on a factually incorrect understanding of the basic meta-learning framework. Additionally, he/she thought our method is based on a pre-trained backbone, which is a clear sign that the reviewer did not read the paper deeply since we propose a meta-adversarial learning approach that enables learning transferable robust representations on unseen domains which does not have any pretraining at all.

Another Reviewer bFkh, gave us a rating of borderline reject with a confidence score of 4 based on nonsensical comments, 1) the absence of an ablation study on loss function, 2) utilization of multiple-view seems to be a basic form of data augmentation. However, we clearly conduct the ablation study on the loss function in Figure 5. Moreover, multi-view augmentation is totally different from data augmentation, where data augmentation is applied in the input while multi-view augmentation is applied through the encoder to generate a different view of task-adaptive parameters during the inner adaptation of the meta-learning. As demonstrated in Table 5, it is hard to achieve robustness on unseen domains with only simple data augmentation. Further, he/she pointed out the complexity of Figure 1 (a), which is an illustration of conventional meta-adversarial learning, not of our main approach. These comments, along with confidence 4, we politely conjecture that Reviewer bFkh may not take the time in reading the whole paper. Thus, the borderline reject rating is unfair and irrational since it is not backed by any factual justification.

During the rebuttal, we did our best to faithfully respond to all questions and comments from all the reviewers, providing the additional experimental results requested by them. We strongly believe that we make an important contribution by proposing novel meta-adversarial learning frameworks with multi-view representation learning for learning transferable robust representations on unseen domains with only a few samples, which is an important yet under-explored problem. Thus we sincerely hope you take the quality of responded reviews into consideration.

Best regards,
Authors



{Final letter to AC, SAC, and PCs}.

Dear AC, SAC, and PCs,

We are writing to express our deep concerns about reviewers (Reviewer bFkh, KeXZ, and bZs8) who have demonstrated critical misunderstanding and factual incorrectness in their understanding of our work, and further have been unresponsive to our clarification. We are deeply disappointed with the quality of the reviews and the irresponsible discussion periods. Therefore, we politely ask ACs to take a look on our responses and please consider the quality of the reviews for a fair evaluation of our work. The following comments summarize the major misunderstanding of each reviewer.

1. Both reviewers bFkh and bZs8 gave our paper a score of 4, claiming that *our work lacks technical novelty as it appears to be a basic form of data augmentation or a simple combination* of meta-learning, adversarial attack, and contrastive learning. 
- However, our method is **fundamentally different from simple data augmentation**, as we suggest generating multi-view by augmenting the whole encoders through the inner adaptation of the meta-learning. We also demonstrated the effectiveness of our approach through ablation experiments in the paper (Table 5). Furthermore, our framework did not employ contrastive learning which is a clear sign of a critical misunderstanding of our work.

2. Reviewer KeXZ changed their score from 6 to 5 without providing specific concerns or suggestions, *claiming that our work lacked novelty in motivation.*
- However, we believe this is an extremely unfair review that may not fully adhere to the guidelines on originality, as it seems to underestimate the novelty of our work. Previous adversarial meta-learning approaches have been limited in their ability to generalize the robustness to unseen domains, following the representation reuse scheme that only focuses on learning the optimal weight of the final classifier. To overcome such limited generalization, **we have a reasonable motivation to leverage representation learning in adversarial meta-learning to obtain transferable robust representation (Line 140)**. We believe we suggest our novel approach with reasonable motivation.

We are truly disappointed with the unjust reviews, where they were not backed up with any justification and were even based on a critical misunderstanding. 
- Our primary contribution is that we are the first to tackle the problem of the limited transferability of the previous meta-adversarial approaches to unseen domains. We believe our work shows **the first attempt to achieve genuine robustness to real-world few-shot tasks**.
- Furthermore, we introduce a **novel meta-adversarial learning framework to obtain transferable robust representations to unseen domains**, which is both an original and creative approach. **The concept of multi-view generation through the inner adaptation** has not been introduced either in meta-learning or self-supervised learning, where our approach can prevent representational collapse without requiring any regularization in contrast to existing SSL methods (Line 197-207). Moreover, by generating adversaries that maximize the discrepancy between two views, we can **explicitly leverage the generalized representation by enforcing the agreements between views and applying individual adversarial loss**, leading to generalized robust representation learning.
- As per the reviewer guidelines, **"originality may arise from creative combinations of existing ideas, application to a new domain,"** and in our case, our work is a novel approach that combines only the concept of multi-view into the meta-learning, even with a unique approach that employs inner adaptation for learning transferable robustness to unseen domains.

Although we have provided detailed responses to correct the reviewers' misunderstandings, we have not received any response from the reviewers yet. We are concerned that the reviewers may conclude **their reviews based on incorrect information and critical misunderstandings**. Thus, we kindly request that you take the quality of the reviews into consideration for a fair evaluation of our work.

We thank you again for your efforts in meta-reviewing our work and ensuring that the review process is fair and constructive.


Sincerely, \
Authors


{Global reminders}
Dear reviewers,

We would like to kindly remind you that we have only a few hours left to address your remaining concerns and discuss them with you. We have taken great care to ensure that we have fully addressed all of your concerns and provided the additional experiments that you requested. For your convenience, we provided a summary of our main contributions and our novelty.

- The main goal of our work is to learn robust and transferable representations for unseen domain tasks in a meta-adversarial learning framework, emphasizing the importance of learning representation rather than representation reuse which is done in previous meta-adversarial learning approaches that showed limited robustness in unseen domains (Line 17, Table 1,2, Line 134-147).

- To achieve learning robust representations, we propose **a novel and unique multi-view augmentation scheme via inner adaptation of meta-learning, generating multi-views by augmenting the entire encoders (Line 33-44, Line 206-219)**. In contrast to self-supervised learning (SSL), our effective multi-view scheme generates the natural discrepancy across the two views through different inner adaptations, preventing the representation collapse that shows the distinct difference compared to SSL (Line 197-207).

- We further propose the **unified optimization objective to learn a generalizable robust representation that is not reliant on tasks or class labels**. We first generate adversaries by maximizing the view discrepancy which is label-free attacks. Then, we enforce the agreements between two views and explicitly regularize each of them with the adversarial loss to ensure robustness on unseen tasks (Line 141-144, 236-259).

- As per the reviewer guidelines, **"originality may arise from creative combinations of existing ideas, application to a new domain,"** and in our case, our work is a novel approach that combines only the concept of multi-view into the meta-learning, even with a unique approach that employs inner adaptation for learning under-explored transferable robustness to unseen domains.

We believe that our contributions demonstrate originality, significance, and creativity. Extensive experimental results demonstrate the effectiveness of our contributions, outperforming the baseline by more than 10\% of robustness. We sincerely hope that you will consider these contributions in your final review and the score.

We thank you again for your valuable time and effort in reviewing our paper and look forward to your feedback.

Best, 
Authors

==> Table/algorithm_bilevel_class.tex <==
\begin{algorithm}[t]
\caption{Transferable robust meta-learning via bilevel class-wise attack}
\begin{algorithmic}
\Require Dataset $\mathbf{D}$, transformation function $t\sim\mathbb{T}$
\Require Encoder $f$, parameter of encoder $\theta$, classifier $h$, parameter of classifier $\mu$ 
\Require adversary $\mathcal{A}$
\While{not done}\\
    Sample tasks $\mathcal{\tau} = (\mathbf{S}(x^s, y^s), \mathbf{Q}(x^q, y^q))$ 
    \For{$\tau = 1, \cdots, $}
            \State transform input $t_1(x^s), t_2(x^s)$
            \State Fine-tune model with $t_1(x^s), t_2(x^s), y^s$ and updates parameter $\theta^{\tau}$
            \State Generate adversarial examples 
            \State $t_1(x^q)^{adv}=\mathcal{A}(t_1(x^q), t_2(x^q), y^q, {\theta^{\tau}})$, $t_2(x^q)^{adv}=\mathcal{A}(t_2(x^q), t_1(x^q), y^q, {\theta^{\tau}})$
            \State Compute gradient $g_i$ = $\nabla_{\theta}\Lagr_{\mathtt{Our}}(h_{\mu}, f_{\theta^{\tau}}, t_1(x^q), t_1(x^q)^{adv}, t_2(x^q), t_2(x^q)^{adv}, y^q)$
    \EndFor
    \State Update model parameters
    \State $\theta, \mu \leftarrow \theta, \mu - \frac{\alpha}{n}\sum g^{\tau}$
\EndWhile
\end{algorithmic}
\label{algo:algorithm_class}
\end{algorithm}


==> Table/algorithm_imageAug.tex <==
\begin{algorithm}[t]
\caption{MAVRL with data augmentation only}
\begin{algorithmic}
\STATE {\bfseries Input:} Dataset $\mathbf{D}$, transformation function $t\sim\mathcal{T}$
\STATE {\bfseries Input:} Encoder $f$ with parameter $\theta$, classifier $h$with parameter $\mu$ 
\STATE {\bfseries Input:} Multi-view latent attack \\$\mathcal{A}(\mathtt{parameter}, \mathtt{base}, \mathtt{target})$
\WHILE{not done}
    \STATE Sample tasks $\{\tau\}$, Support set $\mathbf{S}(x^s, y^s)$, Query set $\mathbf{Q}(x^q, y^q)$ 
    \FOR{$\tau = 1, \cdots, $}
            \STATE Transform input $t_1(x^s), t_2(x^s)$
            \STATE Fine-tune model with $t_1(x^s), t_2(x^s), y^s$ and updates parameter $\theta^{\tau}$
            \STATE Generate adversarial examples 
            \STATE $t_1(x^q)^{adv}=\mathcal{A}({\theta^{\tau}}, t_1(x^q), t_2(x^q))$, $t_2(x^q)^{adv}=\mathcal{A}({\theta^{\tau}}, t_2(x^q), t_1(x^q))$
            \STATE Calculate losses on query set images
            \STATE $\Lagr_{\texttt{adv}_{\theta^{\tau}}} = \Lagr_{\texttt{CE}}(t_1(x^q), y^q) + \Lagr_{\texttt{KL}}(t_1(x^q)^{adv}, t_1(x^q))$
            \STATE $\Lagr_{\texttt{adv}_{\theta^{\tau}}} = \Lagr_{\texttt{CE}}(t_2(x^q), y^q) + \Lagr_{\texttt{KL}}(t_2(x^q)^{adv}, t_2(x^q))$
            \STATE $\Lagr_{\texttt{cos}} = \Lagr_{\texttt{cos}}(z_1^{adv}, z_2^{adv}), z_n^{adv}=f_{\theta^{\tau}}(t_n(x^q)^{adv})$
            \STATE $\Lagr_{\mathtt{Our}} = \Lagr_{\texttt{adv}_{\theta_1^{\tau}}} + \Lagr_{\texttt{adv}_{\theta_2^{\tau}}} + \Lagr_{\texttt{cos}}$
            \STATE Compute gradient $g^{\tau}$ = $\nabla_{\theta^{\tau}}\Lagr_{\mathtt{Our}}$
    \ENDFOR
    \STATE Update model parameters
    \STATE $\theta, \mu \leftarrow \theta, \mu - \frac{\alpha}{\tau}\sum g^{\tau}$
\ENDWHILE
\end{algorithmic}
\label{algo:algorithm_img}
\end{algorithm}

==> Table/app_compareAug_loss.tex <==
% \begin{table}[t]
% \caption{\small Test accuracy(\%) on benchmark data sets for 5-shots. Robustness is calculated with PGD-20 attack($\epsilon=8./255.$, step size=$\epsilon/10$), clean is for clean images. All models are adversarially meta-trained on CIFAR-FS. }
% \centering
% \begin{adjustbox}{width=\textwidth}
%   \begin{tabular}{cclcccccccccc} %
%     \toprule
%     &&&\multicolumn{2}{c}{Mini-ImageNet}&\multicolumn{2}{c}{Tiered-ImageNet}&\multicolumn{2}{c}{CUB}&\multicolumn{2}{c}{Flower}&\multicolumn{2}{c}{Cars}\\
%     \cmidrule(r){4-5}\cmidrule(r){6-7}\cmidrule(r){8-9}\cmidrule(r){10-11}\cmidrule(r){12-13}
%     Data Aug.&Bi-Level Parameter Aug.&Loss&Clean&PGD $\ell_{\infty}$ &Clean& PGD $\ell_{\infty}$&Clean& PGD $\ell_{\infty}$&Clean& PGD $\ell_{\infty}$&Clean& PGD $\ell_{\infty}$\\
%     \midrule
%     % %metasgd, resnet12, attack3
%     -& - & AT~\citep{madry2017pgd}&30.52&18.55&35.54&24.01&39.65&23.20&48.76&35.54&35.16&19.47\\
%     -& - & TRADES~\citep{madry2017pgd}&28.35&17.39&31.73&21.19&34.61&20.46&41.99&30.58&34.42&18.64\\
%     \CheckmarkBold & - &AT~\citep{madry2017pgd}&32.26&16.16&36.47&20.62&36.11&17.44&29.97&14.45\\
%     \CheckmarkBold & - &TRADES~\citep{madry2017pgd}&\\
%     \CheckmarkBold & \CheckmarkBold &AT~\citep{madry2017pgd}&34.61&16.40&38.08&20.45&38.18&17.65&37.11&26.22&32.04&15.53\\
%     \CheckmarkBold & \CheckmarkBold &TRADES~\citep{madry2017pgd}&32.77&19.66&37.92&25.12&40.40&22.45&50.40&43.65&36.73&23.54\\
%     \CheckmarkBold & \CheckmarkBold &AT~\citep{madry2017pgd}+Self-sup&\\
%     \CheckmarkBold & \CheckmarkBold &TRADES~\citep{madry2017pgd}+Self-sup&33.57&16.26&39.26&21.82&39.90&18.62&48.70&36.92&34.69&17.67\\
%     % \multirow{2}{*}{FOMAML}&\CheckmarkBold & - &29.05&15.77&36.17&\textbf{22.03}&31.83&14.30&44.61&34.43&32.40&17.07\\
%     % &\CheckmarkBold & \CheckmarkBold &\textbf{33.57}&\textbf{16.26}&\textbf{39.26}&21.82&\textbf{39.90}&\textbf{18.62}&\textbf{48.70}&\textbf{36.92}&\textbf{34.39}&\textbf{17.67}\\
%     % % %maml, resnet18, attack3
%     % \midrule
%     % %fomaml resnet18, attack3
%     % \multirow{2}{*}{MAML (ResNet18)}&\CheckmarkBold & - &21.84&\textbf{15.49}&25.14&17.89&22.40&13.27&25.09&19.01&22.60&14.36\\
%     % &\CheckmarkBold & \CheckmarkBold & \textbf{36.01}&14.87&\textbf{38.53}&\textbf{18.94}&\textbf{40.29}&\textbf{18.80}&\textbf{57.66}&\textbf{46.85}&\textbf{34.33}&\textbf{16.70} \\
    
    
%     \bottomrule
%   \end{tabular}
%   \label{table:compareAug_Cross}
%   \end{adjustbox}
% \end{table}

\begin{table}[t]
\caption{\small Ablation study on adversarial loss in meta-objectives of MAVRL. Test accuracy(\%) on benchmark data sets for 5-shots. Robustness is calculated with PGD-20 attack ($\epsilon=8./255.$, step size=$\epsilon/10$), clean is for clean images. All models are adversarially meta-trained on CIFAR-FS, with ResNet18 as the base encoder.}
\centering
\begin{adjustbox}{width=\textwidth}
  \begin{tabular}{lcccccccccc} %
    \toprule
    &\multicolumn{2}{c}{Mini-ImageNet}&\multicolumn{2}{c}{Tiered-ImageNet}&\multicolumn{2}{c}{CUB}&\multicolumn{2}{c}{Flower}&\multicolumn{2}{c}{Cars}\\
    \cmidrule(r){2-3}\cmidrule(r){4-5}\cmidrule(r){6-7}\cmidrule(r){8-9}\cmidrule(r){10-11}
    Adversarial Loss&Clean&PGD $\ell_{\infty}$ &Clean& PGD $\ell_{\infty}$&Clean& PGD $\ell_{\infty}$&Clean& PGD $\ell_{\infty}$&Clean& PGD $\ell_{\infty}$\\
    \midrule
    % %metasgd, resnet12, attack3
    % AT~\citep{madry2017pgd}&34.61&16.40&38.08&20.45&38.18&17.65&37.11&26.22&32.04&15.53\\
    % TRADES~\citep{madry2017pgd}&32.77&19.66&37.92&25.12&40.40&22.45&50.40&43.65&36.73&23.54\\
    AT~\citep{madry2017pgd}&\textbf{33.78}&7.99&38.35&12.95&37.00&10.08&42.28&22.19&30.93&9.59\\
    TRADES~\citep{madry2017pgd}&33.57&\textbf{16.26}&\textbf{39.26}&\textbf{21.82}&\textbf{39.90}&\textbf{18.62}&\textbf{48.70}&\textbf{36.92}&\textbf{34.69}&\textbf{17.67}\\
    
    
    \bottomrule
  \end{tabular}
  \vspace{-0.1in}
  \label{table:compareAug_Cross}
  \end{adjustbox}
\end{table}


==> Table/app_table_attack.tex <==
\begin{table}[t]
\caption{\small Test accuracy(\%) on benchmark data sets for 5-shots. Robustness is calculated with PGD-20 attack($\epsilon=8./255.$, step size=$\epsilon/10$), clean is for clean images. All models are adversarially meta-trained on CIFAR-FS. }
\centering
\begin{adjustbox}{width=\textwidth}
  \begin{tabular}{lcccccccccc} %
    \toprule
    &\multicolumn{2}{c}{CIFAR-FS}&\multicolumn{2}{c}{Mini-ImageNet}&\multicolumn{2}{c}{TieredImageNet}&\multicolumn{2}{c}{Flowers}&\multicolumn{2}{c}{Cars}\\
    \cmidrule(r){2-3}\cmidrule(r){4-5}\cmidrule(r){6-7}\cmidrule(r){8-9}\cmidrule(r){10-11}
    Attack type&Clean&Rob. &Clean& Rob.&Clean& Rob.&Clean& Rob.&Clean& Rob.\\
    \midrule %넣어놓고 둘중에 하나 선택하기!
    %meta sgd resnet12
    \textbf{\textit{ResNet12+MetaSGD}} \\
    \:Class-wise  &64.35&	39.88&	40.39&	17.04&	52.65&	27.33&	67.92&	37.58&	39.03&	16.11\\ %cub 결과 49.06	21.25
    \:Bi-level class-wise &66.69&	40.48&	42.15&	17.13&	53.91&	27.41&	69.66&	38.83	&40.05&	16.37 \\%	50.01	21.2
    \:Bi-level instance-wise &65.82&	41.39&	44.64	&15.75	&53.25	&28.05&	70.08&	41.52&	40.08&	16.88\\%	50.78	22.44
    \textbf{\textit{ResNet18+FOMAML}}\\
    %class-wise = augmented single view 1 + trades + attack3
    \:Class-wise & 50.88&35.48&32.90&19.32&37.68&25.02&45.29&33.10&33.14&18.97\\
    \:Bi-level class-wise &53.37&41.04&31.11&20.16&36.98&25.80&51.79&45.98&36.00&23.98\\
    \:Bi-level instance-wise & 64.25&44.96&33.57&16.26&39.26&21.82&48.70&36.92&34.69&17.67\\
    \bottomrule
  \end{tabular}
  \label{table:app_compareAttack}
  \end{adjustbox}
\end{table}


==> Table/app_table_trades_selfsup_loss_compare.tex <==
\begin{table*}[t]
% \begin{minipage} %fomaml resnet18
    \begin{center}
    \caption{\small Experiments results for robust full-finetuning of MAVRL with and without self-supervised loss. Both models are trained on CIFAR-FS, with ResNet18 as the base encoder. Robust accuracy is evaluated with $l_\infty$ PGD-20 attacks with $\epsilon$ = $8./255.$ and the step size $\alpha$ = $8./2550.$, while AA stands for AutoAttack~\citep{croce2020AA}.}    \label{table:selfsup_loss_ablation_full}
    \vspace{-0.1in}
    \resizebox{\linewidth}{!}{
            \begin{tabular}{lcccccccccccc}
            \toprule
            \centering
            &\multicolumn{3}{c}{STL-10} &
            \multicolumn{3}{c}{CARS} & \multicolumn{3}{c}{CUB}&            \multicolumn{3}{c}{AirCraft}\\
            \cmidrule(r){2-4}\cmidrule(r){5-7}\cmidrule(r){8-10}\cmidrule(r){11-13}
            Loss& {Clean} &PGD $\ell_{\infty}$& AA 
             & {Clean} &PGD $\ell_{\infty}$& AA 
             & {Clean} &PGD $\ell_{\infty}$& AA
              & {Clean} &PGD $\ell_{\infty}$& AA \\
              
            \midrule
            {TRADES} %fomaml
            &
            %STL-10
            \textbf{60.41}                                              &
            32.10                                               &
            27.47                                               &
            %CARS
            35.00                                              &
            8.66                                               &
            6.04                                               &
            %CUB
            17.12                                               &
            2.88                                                &
            1.95                                                &
            %AirCraft                                          
            31.79                                               &
            8.07                                                &
            5.22                                               \\
            {TRADES+Self-sup} %fomaml
            &
            %STL-10
            53.46                                              &
            \textbf{32.65}                                               &
            \textbf{28.96}                                               &
            %CARS
            \textbf{31.47}                                              &
            \textbf{9.58}                                               &
            \textbf{6.19}                                               &
            %CUB
            \textbf{18.07}                                               &
            \textbf{4.49}                                               &
            \textbf{2.73}                                               &
            %AirCraft                                       
            \textbf{32.12}                                               &
            \textbf{9.93}                                               &
            \textbf{6.48}                                               \\
            
            \bottomrule
            \end{tabular}        }
    \end{center}
    % \vspace{-0.3in}
\end{table*}

==> Table/my_table.tex <==
\begin{table*}[t]
\caption{\small Results of transferable robustness in 5-way 5-shot unseen domain tasks that are trained on 5-way 5-shot CIFAR-FS and Mini-ImageNet. Rob. stands for accuracy(\%) that is calculated with PGD-20 attack ($\epsilon=8./255.$, step size=$\epsilon/10$). Clean stands for test accuracy(\%) of clean images. All models are trained with PGD-7 attacks on ResNet12.}
\vspace{-0.1in}
\centering
\begin{adjustbox}{width=0.9\textwidth}
    \begin{tabular}{lcccccccccc} %Resnet12, attack7
    \toprule
    &\multicolumn{10}{c}{CIFAR-FS $\rightarrow$}\\
    & \multicolumn{2}{c}{Mini-ImageNet}& \multicolumn{2}{c}{Tiered-ImageNet}&\multicolumn{2}{c}{CUB}&\multicolumn{2}{c}{Flower}& \multicolumn{2}{c}{Cars}\\
    \cmidrule(r){2-11}
    & Clean & Rob.& Clean & Rob.& Clean & Rob. &Clean& Rob.&Clean& Rob.\\
    \midrule
    MAML~\citep{finn2017model} & \underline{44.85}&6.21& \textbf{61.19}&2.48&\underline{48.41}&3.46&\textbf{67.76}&5.73&\textbf{43.94}&5.31 \\
    ADML~\citep{yin2018adml} & 28.66&6.53&40.06&\underline{11.36}&31.18&5.21&39.36&\underline{11.26}&27.43&3.18\\
    
    AQ~\citep{goldblum2020adversarially}&33.09&3.32&37.41&5.05&38.37&4.10&60.14&11.03&36.83&4.47\\
    % AQ r2d2
    %AQ~\citep{goldblum2020adversarially}&36.46&16.10&41.89&21.78&50.97&20.78&75.33&43.36&45.85&20.02\\
    RMAML~\citep{wang2021rmaml}&28.05& \underline{6.65}&29.54&9.30&30.24&\underline{5.67}&42.91&10.79&31.72&\underline{5.56}\\
    Ours&\textbf{45.82}&\textbf{24.12}&	 \underline{51.46}&\textbf{30.06}&\textbf{48.56}&	\textbf{25.23}&\underline{66.49}&\textbf{42.16}&	 \underline{38.29}&\textbf{19.43}\\
    \midrule
    \midrule
    &\multicolumn{10}{c}{Mini-ImageNet $\rightarrow$}\\
    & \multicolumn{2}{c}{CIFAR-FS}& \multicolumn{2}{c}{Tiered-ImageNet}&\multicolumn{2}{c}{CUB}&\multicolumn{2}{c}{Flower}& \multicolumn{2}{c}{Cars}\\
    \cmidrule(r){2-11}
    & Clean & Rob.& Clean & Rob.& Clean & Rob. &Clean& Rob.&Clean& Rob.\\
    \midrule
    MAML~\citep{finn2017model} &\textbf{66.75}&12.97&\textbf{65.33}&13.10&\underline{52.82}&4.46&\textbf{71.01}&4.86&\textbf{43.66}&2.77\\
    ADML~\citep{yin2018adml} &41.14&13.36&41.05&13.26&32.82&4.59&43.07&9.65&24.85&5.48 \\
    AQ~\citep{goldblum2020adversarially}&61.97&\underline{30.73}&47.61&\underline{14.21}&45.64&\underline{13.19}&65.40&\underline{25.01}&37.29&\underline{8.85}\\
    RMAML~\citep{wang2021rmaml}&37.94&10.59&30.49&8.24&27.30&6.26&42.52&13.08&37.76&5.43\\
    Ours&\underline{65.45}&\textbf{36.51}&\underline{59.64}&\textbf{29.73}&\textbf{53.70}&\textbf{20.64}&\underline{69.84}&\textbf{36.49}&\underline{42.25}&\textbf{14.42}\\
    \bottomrule
    \end{tabular}
    \label{table:cifar-crossdomain}
\end{adjustbox}
%\vspace{-0.1in}
\end{table*}


\begin{table*}[t]
\caption{\small Results of transferable robustness in 5-way 5-shot unseen domain tasks that are trained on 5-way 5-shot Mini-ImageNet. Rob. stands for accuracy (\%) that is calculated with PGD-20 attack ($\epsilon=8./255.$, step size=$\epsilon/10$). Clean stands for test accuracy (\%) of clean images. All models are trained with PGD-7 attacks on ResNet12.}
\centering
\vspace{-0.1in}
\begin{adjustbox}{width=0.9\textwidth}
  \begin{tabular}{lcccccccccc} %resnet12, atatck7
    \toprule
    &\multicolumn{10}{c}{Mini-ImageNet $\rightarrow$}\\
    & \multicolumn{2}{c}{CIFAR-FS}& \multicolumn{2}{c}{Tiered-ImageNet}&\multicolumn{2}{c}{CUB}&\multicolumn{2}{c}{Flower}& \multicolumn{2}{c}{Cars}\\
    \cmidrule(r){2-11}
    & Clean & Rob.& Clean & Rob.& Clean & Rob. &Clean& Rob.&Clean& Rob.\\
    \midrule
    MAML~\citep{finn2017model} &\textbf{66.75}&12.97&\textbf{65.33}&13.10&\underline{52.82}&4.46&\textbf{71.01}&4.86&\textbf{43.66}&2.77\\
    ADML~\citep{yin2018adml} &41.14&13.36&41.05&13.26&32.82&4.59&43.07&9.65&24.85&5.48 \\
    AQ~\citep{goldblum2020adversarially}&61.97&\underline{30.73}&47.61&\underline{14.21}&45.64&\underline{13.19}&65.40&\underline{25.01}&37.29&\underline{8.85}\\
    RMAML~\citep{wang2021rmaml}&37.94&10.59&30.49&8.24&27.30&6.26&42.52&13.08&37.76&5.43\\
    Ours&\underline{65.45}&\textbf{36.51}&\underline{59.64}&\textbf{29.73}&\textbf{53.70}&\textbf{20.64}&\underline{69.84}&\textbf{36.49}&\underline{42.25}&\textbf{14.42}\\
    \bottomrule
  \end{tabular}
  \label{table:mini-crossdomain}
  \end{adjustbox}
  \vspace{-0.15in}
\end{table*}



==> Table/table_2.tex <==

\begin{table*}[t]
\caption{\small Results of transferable robustness in 5-way 5-shot unseen domain tasks that are trained on 5-way 5-shot Mini-ImageNet. Rob. stands for accuracy (\%) that is calculated with PGD-20 attack ($\epsilon=8./255.$, step size=$\epsilon/10$). Clean stands for test accuracy (\%) of clean images. All models are trained with PGD-7 attacks on ResNet12.}
\centering
\vspace{-0.1in}
\begin{adjustbox}{width=0.9\textwidth}
  \begin{tabular}{lcccccccccc} %resnet12, atatck7
    \toprule
    &\multicolumn{10}{c}{Mini-ImageNet $\rightarrow$}\\
    & \multicolumn{2}{c}{CIFAR-FS}& \multicolumn{2}{c}{Tiered-ImageNet}&\multicolumn{2}{c}{CUB}&\multicolumn{2}{c}{Flower}& \multicolumn{2}{c}{Cars}\\
    \cmidrule(r){2-11}
    & Clean & Rob.& Clean & Rob.& Clean & Rob. &Clean& Rob.&Clean& Rob.\\
    \midrule
    MAML~\citep{finn2017model} &\textbf{66.75}&12.97&\textbf{65.33}&13.10&\underline{52.82}&4.46&\textbf{71.01}&4.86&\textbf{43.66}&2.77\\
    ADML~\citep{yin2018adml} &41.14&13.36&41.05&13.26&32.82&4.59&43.07&9.65&24.85&5.48 \\
    AQ~\citep{goldblum2020adversarially}&61.97&\underline{30.73}&47.61&\underline{14.21}&45.64&\underline{13.19}&65.40&\underline{25.01}&37.29&\underline{8.85}\\
    RMAML~\citep{wang2021rmaml}&37.94&10.59&30.49&8.24&27.30&6.26&42.52&13.08&37.76&5.43\\
    Ours&\underline{65.45}&\textbf{36.51}&\underline{59.64}&\textbf{29.73}&\textbf{53.70}&\textbf{20.64}&\underline{69.84}&\textbf{36.49}&\underline{42.25}&\textbf{14.42}\\
    \bottomrule
  \end{tabular}
  \label{table:mini-crossdomain}
  \end{adjustbox}
  \vspace{-0.15in}
\end{table*}


==> Table/table_3_4.tex <==
\begin{table}[t]
\centering
% \vspace{-0.1in}
\begin{minipage}{0.48\textwidth}
\caption{\small Results of adversarial robustness for 5-way 5-shot classification tasks on the seen domain. Rob. stands for accuracy (\%) calculated with PGD-20 attack ($\epsilon=8./255.$, $\gamma=\epsilon/10$) $^{*}$ stands for reported results in~\citet{wang2021rmaml}.}
% \vspace{-0.1in}
\begin{adjustbox}{width=\textwidth}
  \begin{tabular}{lcccc} %
    \toprule
    &\multicolumn{2}{c}{CIFAR-FS} &\multicolumn{2}{c}{Mini-ImageNet}\\
    & Clean & Rob.& Clean & Rob.\\
    \midrule
    %attack3, resnet12
    ADML~\citep{yin2018adml}&53.06&22.45&26.72&6.81\\
    %AQ ResNet12
    % AQ~\citep{goldblum2020adversarially}&73.49&28.49&39.47&13.52\\ 
    AQ~\citep{goldblum2020adversarially}&73.19&42.82&36.72&22.89\\
    RMAML~\citep{wang2021rmaml}$^{*}$&57.95&35.30&43.98&21.47 \\
    Ours &64.90&43.34&47.56&18.18 \\
    \bottomrule
  \end{tabular}
  \end{adjustbox}
  \label{table:baseline_result}
 \end{minipage}%
 \hfill
 \begin{minipage}{0.48\textwidth}
 \caption{\small Results of MAVRL with different meta-learning frameworks in 5-way 5-shot few-shot classification tasks on seen domains. All models are trained on CIFAR-FS and Mini-ImageNet, respectively, with PGD-7 attacks on ResNet12.\\}
 \vspace{-0.1in}
 \begin{adjustbox}{width=\textwidth}
  \begin{tabular}{lcccc} %
    \toprule
    &\multicolumn{2}{c}{CIFAR-FS} &\multicolumn{2}{c}{Mini-ImageNet}\\
    & Clean & Rob.& Clean & Rob.\\
    %attack3, resnet12
    \midrule
    MAVRL\\
    \:+MAML~\citep{finn2017model}&52.79&32.50&37.58&14.23\\%maml resnet12, attack3
    \:+FOMAML~\citep{finn2017model} &53.42&35.95&33.87&15.60\\
    \:+Meta-SGD~\citep{li2017meta}&64.90&43.34&47.56&18.18\\ %resnet12
    \bottomrule
  \end{tabular}
\end{adjustbox}
\label{table:metamodel-agnostic}
\end{minipage}%
\end{table}

==> Table/table_5.tex <==
\begin{table*}[t]
%\caption{\small Ablation study of our proposed multi-view augmentation. Test accuracy (\%) on the seen domain (CIFAR-FS) and unseen domains (Mini-ImageNet, Tiered-ImageNet, Cars) of a 5-way 5-shot task. Rob. stands for accuracy(\%) that is calculated with PGD-20 attack ($\epsilon=8./255.$, step size=$\epsilon/10$). Clean stands for test accuracy(\%) of clean images. All models are adversarially meta-trained on CIFAR-FS with attack step $3$ due to computation costs. }
\caption{\small Ablation study of our proposed multi-view encoders for 5-way 5-shot classification tasks on seen and unseen domains. All methods are trained on CIFAR-FS. Rob. stands for accuracy (\%) that is calculated with PGD-20 attack ($\epsilon=8./255.$, $\gamma=\epsilon/10$).}
\vspace{-0.1in}
\centering
\begin{adjustbox}{width=0.95\linewidth}
  \begin{tabular}{cc cc cc cc cc cc cc} %
    \toprule
    \multicolumn{2}{c}{Augmentation Type}&\multicolumn{2}{c}{CIFAR-FS}&\multicolumn{2}{c}{Mini-ImageNet}&\multicolumn{2}{c}{Tiered-ImageNet}&\multicolumn{2}{c}{Flower}&\multicolumn{2}{c}{Cars}&\multicolumn{2}{c}{CUB}\\
    \cmidrule(r){1-2}\cmidrule(r){3-4}\cmidrule(r){5-6}\cmidrule(r){7-8}\cmidrule(r){9-10}\cmidrule(r){11-12}\cmidrule(r){13-14}
    Data Aug.&Multi-view Enc.&Clean&Rob. &Clean& Rob.&Clean& Rob.&Clean& Rob.&Clean& Rob.&Clean& Rob.\\
    \midrule
    \checkmark & - &64.35 & 39.88 & 40.39 & \textbf{17.04} & 52.65 & 27.33 & 67.92 & 37.58 & 39.03 & 16.11 & 49.06 & 21.25\\
    %
    \checkmark & \checkmark &\textbf{65.82}&	\textbf{41.39}&	\textbf{44.64}	&15.75	&\textbf{53.25}	&\textbf{28.05}&	\textbf{70.08}&	\textbf{41.52}&	\textbf{40.08}	&\textbf{16.88}&\textbf{50.78}&	\textbf{22.44}
\\
    \bottomrule
  \end{tabular}
  \label{table:compareAug}
  \vspace{-0.1in}
\end{adjustbox}
\end{table*}




==> Table/table_6.tex <==
\begin{table*}[t]
%\caption{\small Ablation study of our proposed multi-view latent attack. Test accuracy(\%) on the seen domain (CIFAR-FS) and unseen domains (Mini-ImageNet, Tiered-ImageNet, Flower, CUB) of a 5-way 5-shot task. Rob. stands for accuracy(\%) that is calculated with PGD-20 attack ($\epsilon=8./255.$, step size=$\epsilon/10$). Clean stands for test accuracy(\%) of clean images. All models are adversarially meta-trained on CIFAR-FS with attack step $3$ due to computation costs.}
\vspace{-0.1in}
\caption{\small Ablation study of our proposed attack type for 5-way 5-shot classification tasks on seen and unseen domains. All methods are trained on CIFAR-FS. Rob. stands for accuracy (\%) that is calculated with PGD-20 attack ($\epsilon=8./255.$, $\gamma=\epsilon/10$).}
\vspace{-0.1in}
\centering
\begin{adjustbox}{width=0.95\linewidth}
  \begin{tabular}{lcccccccccccc} %
    \toprule
    &\multicolumn{2}{c}{CIFAR-FS}&\multicolumn{2}{c}{Mini-ImageNet}&\multicolumn{2}{c}{Tiered-ImageNet}&\multicolumn{2}{c}{Flower}&\multicolumn{2}{c}{Cars}&\multicolumn{2}{c}{CUB}\\
    \cmidrule(r){2-3}\cmidrule(r){4-5}\cmidrule(r){6-7}\cmidrule(r){8-9}\cmidrule(r){10-11}\cmidrule(r){12-13}
    Attack Type&Clean&Rob. &Clean& Rob.&Clean& Rob.&Clean& Rob.&Clean& Rob.&Clean& Rob.\\
    \midrule 
    Class-wise attack &\textbf{66.69}&	40.48&	42.15&\textbf{	17.13}&	\textbf{53.91}&	27.41&	69.66&	38.83	&40.05	&16.37&	50.01&	21.20\\
    Multi-view latent attack &65.82&	\textbf{41.39}&	\textbf{44.64}	&15.75	&53.25	&\textbf{28.05}&	\textbf{70.08}&	\textbf{41.52}&	\textbf{40.08}	&\textbf{16.88}&\textbf{50.78}&	\textbf{22.44}\\
    \bottomrule
  \end{tabular}
  \label{table:compareAttack}
  \end{adjustbox}
  \vspace{-0.25in}
\end{table*}


==> Table/table_7.tex <==
\begin{table*}[t]
% \begin{minipage}
    \begin{center}
    \caption{\small Experiments results in robust full-finetuning of MAVRL and the state-of-the-art adversarial self-supervised learning (SSL) models. While MAVRL is trained on CIFAR-FS, other models are trained on the CIFAR-100. MAVRL is pre-trained with parameter-augmented latent attacks with 3 steps due to computational overhead, others are pre-trained with PGD-7 attacks. All models are trained on ResNet18. We evaluate all models with PGD-20 steps and AutoAttack (AA)~\citep{croce2020AA} with $\epsilon$=8/255.}
    \label{table:table_transfer}
    \vspace{-0.1in}
    \begin{adjustbox}{width=\textwidth}
            \begin{tabular}{clccccccccc}
            \toprule
            \centering
            % % &\multicolumn{6}{c}{Unseen domain} & \multicolumn{3}{c}{Seen domain}\\
            % \cmidrule(r){2-7}\cmidrule(r){8-10}
            &&\multicolumn{3}{c}{CIFAR-10} & \multicolumn{3}{c}{STL-10}&            \multicolumn{3}{c}{CIFAR-100}\\
            \cmidrule(r){3-5}\cmidrule(r){6-8}\cmidrule(r){9-11}
            &Method& {Clean} &PGD-20& AA 
            
             & {Clean} &PGD-20& AA 
             
              & {Clean} &PGD-20& AA \\
            \midrule
            % \textbf{\textit{Self-supervised learning}} \\
            \multirow{3}{*}{\rotatebox[origin=c]{90}{\small SSL}}&{\:RoCL~\citep{kim2020rocl}}
            &
            %CIFAR10
            76.76                                              &
            50.72                                               &
            45.52                                               &
            %STL10
            60.44                                               &
            31.90                                               &
            27.38                                               &
            %CIFAR100                                           
            51.91                                               &
            27.77                                               &
            22.79                                               \\
            &{\:ACL~\citep{jiang2020ACL}}                           &
            %CIFAR10
            75.99                                              &
            50.35                                               &
            45.50                                               &
            %STL10
            63.46                                               &
            30.24                                               &
            25.73                                               &
            %CIFAR100                                           
            51.91                                               &
            27.77                                               &
            22.79                                               \\
            &{\:BYORL~\citep{gowal2020self}}                        &
            76.39                                               &
            50.51                                               &
            45.37                                               &
            %STL10
            62.85                                               &
            28.15                                               &
            24.23                                               &
            %CIFAR100                                           
            52.37                                               &
            28.09                                               &
            23.11                                               \\
            % \textbf{\textit{Meta learning}} \\
            
            &\textbf{\:Ours (3 steps)}                                       &
            %CIFAR10 %fomaml resnet18, attack7
            74.26                                               &
            49.38                                               &
            44.31                                               &
            %STL10
            53.46                                               &
            32.65                                               &
            28.96                                               &
            %CIFAR100
            50.23                                               &
            27.05                                               &
            21.96                                               \\
            % \textbf{\:Ours (7 steps)}                           &
            % %CIFAR10 %fomaml resnet18, attack7
            % 74.31                                               &
            % 49.59                                               &
            % 44.55                                               &
            % %STL10
            % 56.69                                               &
            % 32.13                                               &
            % 28.33                                               &
            % %CIFAR100
            % 50.05                                               &
            % 27.14                                               &
            % 22.05                                               \\
            \bottomrule
            
            \end{tabular}        
            \end{adjustbox}
    
    \end{center}
    \vspace{-0.15in}
\end{table*}

% \begin{table*}[t]
% % \begin{minipage}
%     \begin{center}
%     \caption{\small Experiments results in robust full-finetuning of MAVRL and the state-of-the-art adversarial self-supervised models. While MAVRL is trained on CIFAR-FS, other models are trained on the full-dataset of CIFAR-100. All models are evaluated against PGD-20 attacks ($\epsilon$ = $8./255.$) and AutoAttack (AA)~\citep{croce2020AA}. While MAVRL is pre-trained with bilevel attacks with 3 steps, others are pre-traiend with PGD-7 attacks.}
%     \label{table:table_transfer}
%     \vspace{-0.1in}
%     \begin{adjustbox}{width=\textwidth}
%             \begin{tabular}{lccccccccc}
%             \toprule
%             \centering
%             &\multicolumn{6}{c}{Unseen domain} & \multicolumn{3}{c}{Seen domain}\\
%             \cmidrule(r){2-7}\cmidrule(r){8-10}
%             &\multicolumn{3}{c}{CIFAR-10} & \multicolumn{3}{c}{STL-10}&            \multicolumn{3}{c}{CIFAR-100}\\
%             \cmidrule(r){2-4}\cmidrule(r){5-7}\cmidrule(r){8-10}
%             Method& {Clean} &PGD-20& AA 
            
%              & {Clean} &PGD-20& AA 
             
%               & {Clean} &PGD-20& AA \\
%             \midrule
%             \textbf{\textit{Self-supervised learning}} \\
%             {\:RoCL~\citep{kim2020rocl}}
%             &
%             %CIFAR10
%             76.76                                              &
%             50.72                                               &
%             45.52                                               &
%             %STL10
%             60.44                                               &
%             31.90                                               &
%             27.38                                               &
%             %CIFAR100                                           
%             51.91                                               &
%             27.77                                               &
%             22.79                                               \\
%             {\:ACL~\citep{jiang2020ACL}}                           &
%             %CIFAR10
%             75.99                                              &
%             50.35                                               &
%             45.50                                               &
%             %STL10
%             63.46                                               &
%             30.24                                               &
%             25.73                                               &
%             %CIFAR100                                           
%             51.91                                               &
%             27.77                                               &
%             22.79                                               \\
%             {\:BYORL~\citep{gowal2020self}}                        &
%             76.39                                               &
%             50.51                                               &
%             45.37                                               &
%             %STL10
%             62.85                                               &
%             28.15                                               &
%             24.23                                               &
%             %CIFAR100                                           
%             52.37                                               &
%             28.09                                               &
%             23.11                                               \\
%             \textbf{\textit{Meta learning}} \\
            
%             \textbf{\:Ours (3 steps)}                                       &
%             %CIFAR10 %fomaml resnet18, attack7
%             74.26                                               &
%             49.38                                               &
%             44.31                                               &
%             %STL10
%             53.46                                               &
%             32.65                                               &
%             28.96                                               &
%             %CIFAR100
%             50.23                                               &
%             27.05                                               &
%             21.96                                               \\
%             % \textbf{\:Ours (7 steps)}                           &
%             % %CIFAR10 %fomaml resnet18, attack7
%             % 74.31                                               &
%             % 49.59                                               &
%             % 44.55                                               &
%             % %STL10
%             % 56.69                                               &
%             % 32.13                                               &
%             % 28.33                                               &
%             % %CIFAR100
%             % 50.05                                               &
%             % 27.14                                               &
%             % 22.05                                               \\
%             \bottomrule
            
%             \end{tabular}        
%             \end{adjustbox}
    
%     \end{center}
%     \vspace{-0.1in}
% \end{table*}



% \begin{table*}[t]
% % \begin{minipage}
%     \begin{center}
%     \caption{\small Experiments results for self-supervised linear and robust linear evaluation of SAML and the state-of-the-art robust self-supervised models. While SAML trained on CIFAR-FS, other models are trained on full-dataset of CIFAR-100.}    \label{table:table_transfer}
%     \vspace{-0.1in}
%     \resizebox{\linewidth}{!}{
%             \begin{tabular}{c|c|l|ccc}
%             \toprule
%             \centering
%             % \multicolumn{1}{c}{\multirow{2}{*}{Device}} &
%             \multirow{2}{*}{Target Data} &
%             \multicolumn{1}{c|}{\multirow{2}{*}{Train type}} & {\multirow{2}{*}{Self-supervised\\ framework}} &  \multicolumn{3}{c}{Accuracy} \\
%             & & & {Clean} &PGD $\ell_{\infty}$& AutoAttack \\
%             \midrule
%             \midrule
%             \multirow{4}{*}{CIFAR-10}                           &
%             \multirow{4}{*}{\makecell{Robust transfer learning}} & 
%             {ACL~\cite{jiang2020ACL}}                           &
%             75.99                                              &
%             50.35                                               &
%             45.50                                               \\
%                                                                 &
%                                                                 & 
%             {BYORL~\cite{gowal2020self}}                        &
%             76.39                                               &
%             50.51                                               &
%             45.37                                               \\
%                                                                 &
%                                                                 &  
%             {AQ~\cite{goldblum2020adversarially}}               &
%             73.15                                              &
%             48.16                                               &
%             43.40                                              \\
%                                                                 &
%                                                                 & 
%             \textbf{Ours}                                       &
%             75.10                                               &
%             49.77                                               &
%             44.78                                               \\
%             \midrule
%             \multirow{4}{*}{STL-10}                              &
%             \multirow{4}{*}{\makecell{Robust transfer learning}} & 
%             {ACL~\cite{jiang2020ACL}}                           &
%             63.46                                               &
%             30.24                                               &
%             25.73                                               \\
%                                                                 &
%                                                                 & 
%             {BYORL~\cite{gowal2020self}}                        &
%             62.85                                               &
%             28.15                                               &
%             24.23                                               \\
%                                                                 &
%                                                                 &  
%             {AQ~\cite{goldblum2020adversarially}}               &
%             62.21                                               &
%             31.04                                               &
%             26.73                                               \\
%                                                                 &
%                                                                 & 
%             \textbf{Ours}                                       &
%             58.96                                               &
%             31.60                                               &
%             27.08                                               \\
%             \bottomrule
%             \end{tabular}        }
%     \end{center}
%     \vspace{-0.1in}
% \end{table*}

% \begin{table*}[t]
% % \begin{minipage}
%     \begin{center}
%     \caption{\small Experiments results for self-supervised linear and robust linear evaluation of SAML and the state-of-the-art robust self-supervised models. While SAML trained on CIFAR-FS, other models are trained on full-dataset of CIFAR-100.}    \label{table:table_transfer}
%     \vspace{-0.1in}
%     \resizebox{\linewidth}{!}{
%             \begin{tabular}{c|c|l|ccc}
%             \toprule
%             \centering
%             % \multicolumn{1}{c}{\multirow{2}{*}{Device}} &
%             \multirow{2}{*}{Target Data} &
%             \multicolumn{1}{c|}{\multirow{2}{*}{Train type}} & {\multirow{2}{*}{Self-supervised\\ framework}} &  \multicolumn{3}{c}{Accuracy} \\
%             & & & {Clean} &PGD $\ell_{\infty}$& AutoAttack \\
%             \midrule
%             \midrule
%             \multirow{12}{*}{CIFAR-10}                           &
%             \multirow{4}{*}{\makecell{Self-supervised\\ linear evaluation}} &  
%             {ACL~\cite{jiang2020ACL}}                           &
%             52.79                                               &
%             17.40                                               &
%             14.32                                               \\
%                                                                 &
%                                                                 &  
%             {BYORL~\cite{gowal2020self}}                        &
%             71.06                                               &
%             16.57                                               &
%             2.10                                               \\
%                                                                 &
%                                                                 &  
%             {AQ~\cite{goldblum2020adversarially}}               &
%             60.34                                               &
%             7.45                                                &
%             4.94                                              \\
%                                                                 &
%                                                                 & 
%             \textbf{Ours}                                       &
%             37.98                                               &
%             15.79                                               &
%             9.59                                               \\
%             \cdashline{2-6}\noalign{\vskip 0.75ex}
%                                                                 &
%             \multirow{4}{*}{\makecell{Self-supervised\\ robust linear evaluation}} & 
%             {ACL~\cite{jiang2020ACL}}                           &
%             46.62                                               &
%             29.17                                               &
%             23.06                                               \\
%                                                                 &
%                                                                 & 
%             {BYORL~\cite{gowal2020self}}                        &
%             56.39                                               &
%             34.42                                                &
%             13.94                                               \\
%                                                                 &
%                                                                 &  
%             {AQ~\cite{goldblum2020adversarially}}               &
%             40.88                                               &
%             21.47                                               &
%             11.20                                               \\
%                                                                 &
%                                                                 & 
%             \textbf{Ours}                                       &
%             34.77                                               &
%             21.21                                               &
%             10.82                                               \\
%             \cdashline{2-6}\noalign{\vskip 0.75ex}
%                                                                 &
%             \multirow{4}{*}{\makecell{Robust transfer learning}} & 
%             {ACL~\cite{jiang2020ACL}}                           &
%             75.99                                              &
%             50.35                                               &
%             45.50                                               \\
%                                                                 &
%                                                                 & 
%             {BYORL~\cite{gowal2020self}}                        &
%             76.39                                               &
%             50.51                                               &
%             45.37                                               \\
%                                                                 &
%                                                                 &  
%             {AQ~\cite{goldblum2020adversarially}}               &
%             73.15                                              &
%             48.16                                               &
%             43.40                                              \\
%                                                                 &
%                                                                 & 
%             \textbf{Ours}                                       &
%             75.10                                               &
%             49.77                                               &
%             44.78                                               \\
%             \midrule
%             \multirow{12}{*}{STL-10}                              &
%             \multirow{4}{*}{\makecell{Self-supervised \\ linear evaluation}} &  
%             {ACL~\cite{jiang2020ACL}}                           &
%             46.39                                               &
%             20.69                                               &
%             17.58                                               \\
%                                                                 &
%                                                                 &  
%             {BYORL~\cite{gowal2020self}}                        &
%             63.53                                               &
%             12.93                                               &
%             2.43                                               \\
%                                                                 &
%                                                                 &  
%             {AQ~\cite{goldblum2020adversarially}}               &
%             53.19                                               &
%             7.26                                                &
%             4.56                                               \\
%                                                                 &
%                                                                 & 
%             \textbf{Ours}                                       &
%             33.19                                               &
%             15.71                                               &
%             5.13                                                \\
%             \cdashline{2-6}\noalign{\vskip 0.75ex}
%                                                                 &
%             \multirow{4}{*}{\makecell{Self-supervised\\ robust linear evaluation}} & 
%             {ACL~\cite{jiang2020ACL}}                           &
%             43.05                                               &
%             27.02                                               &
%             22.66                                               \\
%                                                                 &
%                                                                 & 
%             {BYORL~\cite{gowal2020self}}                        &
%             54.23                                                &
%             32.05                                               &
%             12.53                                               \\
%                                                                 &
%                                                                 &  
%             {AQ~\cite{goldblum2020adversarially}}               &
%             45.2
%                 &
%             19.5
%                 &
%             10.63                                               \\
%                                                                 &
%                                                                 & 
%             \textbf{Ours}                                       &
%             28.76                                               &
%             18.86                                               &
%             8.19                                               \\
%             \cdashline{2-6}\noalign{\vskip 0.75ex}
%                                                                 &
%             \multirow{4}{*}{\makecell{Robust transfer learning}} & 
%             {ACL~\cite{jiang2020ACL}}                           &
%             63.46                                               &
%             30.24                                               &
%             25.73                                               \\
%                                                                 &
%                                                                 & 
%             {BYORL~\cite{gowal2020self}}                        &
%             62.85                                               &
%             28.15                                               &
%             24.23                                               \\
%                                                                 &
%                                                                 &  
%             {AQ~\cite{goldblum2020adversarially}}               &
%             62.21                                               &
%             31.04                                               &
%             26.73                                               \\
%                                                                 &
%                                                                 & 
%             \textbf{Ours}                                       &
%             58.96                                               &
%             31.60                                               &
%             27.08                                               \\
%             \bottomrule
%             \end{tabular}        }
%     \end{center}
%     \vspace{-0.1in}
% \end{table*}


==> Table/table_compareCleanMaml.tex <==
% \begin{table}[t]
% \caption{\small Test accuracy(\%) of 5-shots trained models on CIFAR-FS on unseen domain adaptation. Robustness is calculated with PGD-20 attack ($\epsilon=8./255.$, step size=$\epsilon/10$), clean stands for accuracy of clean images. All models are trained with PGD-7 attacks ($\epsilon=8./255.$, step size=$2./255.$) on ResNet12.}
% \centering
% \begin{adjustbox}{width=\textwidth}
%   \begin{tabular}{lcccccccccc} 
%     \toprule
%     &\multicolumn{10}{c}{CIFAR-FS $\rightarrow$}\\ \multicolumn{2}{c}{mini-ImageNet}& \multicolumn{2}{c}{tiered-ImageNet}&\multicolumn{2}{c}{CUB}&\multicolumn{2}{c}{Flowers}& \multicolumn{2}{c}{Cars}\\
%     \cmidrule(r){2-11}
%     & Clean & Rob.& Clean & Rob.& Clean & Rob. &Clean& Rob.&Clean& Rob.\\
%     \midrule
%     MAML~\citep{finn2017model} &44.85&6.21&61.19&2.48&48.41&3.46&67.76&5.73&43.94&5.31\\
%     TROBA$_{clean(CE)}$&39.80&0.23&42.58&0.58&45.63&0.51&70.00&1.60&43.59&0.31\\
%     TROBA$_{clean(CE+Self-sup)}$&41.51&0.49&42.82&0.62&47.58&0.49&71.98&2.41&43.23&0.78\\
%     \bottomrule
%   \end{tabular}
%   \label{table:clean_maml}
% \end{adjustbox}
% \end{table}

==> Table/table_loss_ablation.tex <==
\begin{table}[t]
\caption{\small Test accuracy(\%) on benchmark data sets for 5-shots. Robustness is calculated with PGD-20 attack($\epsilon=8./255.$, step size=$\epsilon/10$), clean is for clean images. All models are adversarially meta-trained on CIFAR-FS. }
\centering
\begin{adjustbox}{width=\textwidth}
  \begin{tabular}{ccc cc cc cc cc} %
    \toprule
    \multicolumn{3}{c}{\textbf{Loss}}&\multicolumn{2}{c}{\textbf{In-domain}}&\multicolumn{6}{c}{ \textbf{Cross-domain}}\\
    \cmidrule(r){1-3}\cmidrule(r){4-5}\cmidrule(r){6-11}
    \multicolumn{2}{c}{$\Lagr_{\texttt{TRADES}}$}&&\multicolumn{2}{c}{CIFAR-FS}&\multicolumn{2}{c}{Mini-ImageNet}&\multicolumn{2}{c}{TieredImageNet}&\multicolumn{2}{c}{Cars}\\
    \cmidrule(r){1-2}\cmidrule(r){4-5}\cmidrule(r){6-7}\cmidrule(r){8-9}\cmidrule(r){10-11}
    $\Lagr_{\texttt{CE}}$&$\Lagr_{\texttt{KL}}$&$\Lagr_{\texttt{selfsup}}$&Clean&PGD $\ell_{\infty}$ &Clean& PGD $\ell_{\infty}$&Clean& PGD $\ell_{\infty}$&Clean& PGD $\ell_{\infty}$\\
    \midrule
    \CheckmarkBold & - & - &48.06&14.13&26.51&6.07&29.37&7.74&27.81&8.76\\
    \CheckmarkBold & - & \CheckmarkBold & 41.86 & 16.21 & 24.95 & 5.98 & 28.15 &7.59&24.28&10.43\\
    \CheckmarkBold & \CheckmarkBold & - & 52.28 & 36.50 & 32.77 & 19.66 & 37.92 &25.12&36.73&23.54\\
    \CheckmarkBold & \CheckmarkBold & \CheckmarkBold&64.25&44.96&33.57&16.26&39.26&21.82&34.69&17.67\\
    \bottomrule
  \end{tabular}
  \label{table:compareAug}
  \end{adjustbox}
\end{table}

==> Table/table_metaTest.tex <==
\begin{table}[t]
\caption{\small Test accuracy(\%) on benchmark data sets for 5-shots. Robustness is calculated with PGD-20 attack($\epsilon=8./255.$, step size=$\epsilon/10$), clean is for clean images. Both SAML and AQ are trained on CIFAR-FS. }
\centering
  \begin{tabular}{lccccc} %
    \toprule
    &\multicolumn{2}{c}{AQ~\citep{goldblum2020adversarially}}&\multicolumn{2}{c}{Ours}\\
    \cmidrule(r){2-3}\cmidrule(r){4-5}
    Meta-test & Clean & PGD $\ell_{\infty}$ &Clean& PGD $\ell_{\infty}$ \\
    \midrule
    \textit{\textbf{In-domain}} \\
    CIFAR-FS &76.19&36.94&\\
    \textit{\textbf{Cross-domain}}\\
    MiniImageNet&37.98&11.96 \\
    TieredImageNet&43.08&17.54 \\
    CARS&46.73&14.49 \\
    AirCraft&40.91&9.49 \\
    VggFlower&76.31&36.49 \\
    \bottomrule
  \end{tabular}
  \label{table:table5}
\end{table}

==> Table/table_metaTest_cross_domain.tex <==
\begin{table}[t]
\caption{\small Test accuracy(\%) on benchmark data sets for 5-shots. Robustness is calculated with PGD-20 attack($\epsilon=8./255.$, step size=$\epsilon/10$), clean is for clean images. Both SAML and AQ are trained on CIFAR-FS. }
\centering
\begin{adjustbox}{width=0.8\textwidth}
  \begin{tabular}{lccccc} %
    \toprule
    &&\multicolumn{2}{c}{AQ~\citep{goldblum2020adversarially}}&\multicolumn{2}{c}{Ours}\\
    \cmidrule(r){3-4}\cmidrule(r){5-6}
    Meta-train&Meta-test & Clean & PGD $\ell_{\infty}$ &Clean& PGD $\ell_{\infty}$ \\
    \midrule
    \multirow{4}{*}{CIFAR-FS}&MiniImageNet&34.56&4.86&35.61&\textbf{20.61} \\
    &TieredImageNet&38.94&8.75&40.83&\textbf{26.33} \\
    &CARS&40.18&5.29&38.97&\textbf{22.37} \\
    &AirCraft&36.07&3.84&31.4&\textbf{17.18} \\
    \bottomrule
  \end{tabular}
  \label{table:cross_domain_result}
\end{adjustbox}
\end{table}

==> Table/table_metaTest_crossdomain_miniImagenet.tex <==
\begin{table}[t]
\caption{\small Test accuracy(\%) on benchmark data sets for 5-shots. Robustness is calculated with PGD-20 attack($\epsilon=8./255.$, step size=$\epsilon/10$), clean is for clean images. Both SAML and AQ are trained on miniImageNet. }
\centering
\begin{adjustbox}{width=0.8\textwidth}
  \begin{tabular}{lccccc} %
    \toprule
    &&\multicolumn{2}{c}{AQ~\citep{goldblum2020adversarially}}&\multicolumn{2}{c}{Ours}\\
    \cmidrule(r){3-4}\cmidrule(r){5-6}
    Meta-train&Meta-test & Clean & PGD $\ell_{\infty}$ &Clean& PGD $\ell_{\infty}$ \\
    \midrule
    \multirow{5}{*}{miniImageNet}&TieredImageNet&44.22&18.45&41.3&\textbf{20.23}\\
    &CARS&40.98&7.87&41.18&\textbf{14.97}\\
    &AirCraft&33.97&5.54&29.56&\textbf{11.99}\\
    &FC100&54.93&18.48&45.88&\textbf{19.63}\\
    &CIFAR-FS&72.74&34.44&60.76&\textbf{35.21}\\
    \bottomrule
  \end{tabular}
  \label{table:cross_domain_result_mini}
\end{adjustbox}
\end{table}

% \begin{wraptable}[8]{r}{7.0cm}
% \vspace{-0.2in}
% \caption{\small Ablation experiments on score function ($\mathcal{S}$). }
% \centering
% \vspace{-0.13in}
%   \begin{tabular}{ccc|cc} %
%     \toprule
%     Similarity & Entropy & KL-div& Clean & Rob.\\
%     \midrule
%     \checkmark & - & -\\
%     \checkmark & \checkmark & -\\
%     \checkmark & - & \checkmark\\
%     \checkmark & \checkmark & \checkmark\\
%     \multicolumn{3}{c}{Random Selection}& \\
%     \bottomrule
%   \end{tabular}
%   \label{table:ablation_score_function}
% \end{wraptable}

==> Table/table_metatest_crossdomain_combined.tex <==
\begin{table}[t]
\caption{\small Test accuracy(\%) on benchmark data sets for 5-shots. Robustness is calculated with PGD-20 attack($\epsilon=8./255.$, step size=$\epsilon/10$), clean is for clean images. Both SAML and AQ are trained on CIFAR-FS. }
\centering
\begin{adjustbox}{width=\textwidth}
  \begin{tabular}{lcccclcccc} %
    \toprule
    &\multicolumn{4}{c}{CIFAR-FS}&&\multicolumn{4}{c}{MiniImageNet}\\
    \cmidrule(r){2-5}\cmidrule(r){7-10}
    & \multicolumn{2}{c}{AQ}& \multicolumn{2}{c}{Ours}&& \multicolumn{2}{c}{AQ}&\multicolumn{2}{c}{Ours}\\
    & Clean & PGD $\ell_{\infty}$& Clean & PGD $\ell_{\infty}$&& Clean & PGD $\ell_{\infty}$ &Clean& PGD $\ell_{\infty}$ \\
    \midrule
    MiniImageNet&34.56&4.86&33.57&16.26&CIFAR-FS&72.74&34.44&58.27&34.
    4\\
    TieredImageNet&38.94&8.75&39.26&21.82&TieredImageNet&44.22&18.45&39.67&19.27 \\
    CARS&40.18&5.29&34.69&17.67&CARS&40.98&7.87&38.46&14.41\\
    AirCraft&36.07&3.84&29.72&14.34&AirCraft&33.97&5.54&28.26&11.33\\
    CUB&44.21&5.66&40.88&16.37&CUB&51.03&12.48&40.88&16.37 \\
    \bottomrule
  \end{tabular}
  \label{table:cross_domain_results_combined}
\end{adjustbox}
\end{table}

==> Table/table_wrap_rocl.tex <==
\begin{table}[t]
\caption{\small Results of transferable robustness in 5-shots unseen domain tasks. TROBA is trained on CIFAR-FS, with ResNet18 as the base encoder. On top of the pre-trained ROCL, we meta-train the model for 300 epochs as the same environment as TROBA is trained. Rob. stands for accuracy(\%) that is calculated with PGD-20 attack ($\epsilon=8./255.$, step size=$\epsilon/10$). Clean stands for test accuracy(\%) of clean images.}
\centering
\vspace{-0.1in}
\begin{adjustbox}{width=\textwidth}
  \begin{tabular}{lcccccccccc} %
    \toprule
    & \multicolumn{2}{c}{mini-ImageNet}& \multicolumn{2}{c}{Tiered-ImageNet}&\multicolumn{2}{c}{CUB}&\multicolumn{2}{c}{Flowers}& \multicolumn{2}{c}{Cars}\\
    \cmidrule(r){2-11}
    & Clean & Rob.& Clean & Rob.& Clean & Rob. &Clean& Rob.&Clean& Rob.\\
    \midrule
    TROBA&33.57&16.26&39.26&21.82&39.90&18.62&48.70&36.92&34.69&17.67 \\
    ROCL~\citep{kim2020rocl}+TROBA &40.87&21.35&45.68&26.47&39.74&20.15&32.25&22.12&28.07&15.80 \\
    \bottomrule
  \end{tabular}
  \label{table:rocl}
\end{adjustbox}
\end{table}
